rETF-semiSL: Semi-Supervised Learning for Neural Collapse in Temporal Data

Deep neural networks for time series must capture complex temporal patterns, to effectively represent dynamic data. Self- and semi-supervised learning methods show promising results in pre-training large models, which -- when finetuned for classification -- often outperform their counterparts trained from scratch. Still, the choice of pretext training tasks is often heuristic and their transferability to downstream classification is not granted, thus we propose a novel semi-supervised pre-training strategy to enforce latent representations that satisfy the Neural Collapse phenomenon observed in optimally trained neural classifiers. We use a rotational equiangular tight frame-classifier and pseudo-labeling to pre-train deep encoders with few labeled samples. Furthermore, to effectively capture temporal dynamics while enforcing embedding separability, we integrate generative pretext tasks with our method, and we define a novel sequential augmentation strategy. We show that our method significantly outperforms previous pretext tasks when applied to LSTMs, transformers, and state-space models on three multivariate time series classification datasets. These results highlight the benefit of aligning pre-training objectives with theoretically grounded embedding geometry.

==> tables/tab_results.tex <==
\begin{tabular}{lr@{ \textpm }lr@{ \textpm }l}
\toprule
\scshape Model and properties & \multicolumn{2}{r}{\scshape Classification F1} & \multicolumn{2}{r}{\scshape Detection AUROC} \\
\midrule
\itshape CNN-LSTM & 0.617 & 0.023 & 0.755 & 0.010 \\
\itshape LSTM & 0.650 & 0.080 & 0.767 & 0.026 \\
\midrule
\itshape Dist-DCRNN & 0.717 & 0.074 & 0.856 & 0.008 \\
\itshape Dist-DCRNN + SSL & 0.729 & 0.023 & 0.860 & 0.015 \\
\midrule
\itshape GTS & 0.710 & 0.050 & 0.856 & 0.020 \\
\itshape ${}^*$WGTS & 0.716 & 0.036 & 0.822 & 0.031 \\
\itshape ${}^*$WGTS + dist & 0.710 & 0.036 & 0.845 & 0.016 \\
\itshape ${}^*$WGTS + SSL & \underline{0.762} & \underline{0.013} & 0.847 & 0.003 \\
\itshape ${}^*$WGTS + SSL + dist & 0.753 & 0.035 & \underline{0.861} & \underline{0.013} \\
% \itshape ${}^*$WGTS + SSL + data-agnostic & 0.747 & 0.058 & 0.848 & 0.023 \\
\midrule
\itshape ${}^*$WGTS Dynamic & 0.737 & 0.062 & 0.843 & 0.008 \\
\itshape ${}^*$WGTS Dynamic + dist & 0.735 & 0.025 & \bfseries 0.867 & \bfseries 0.007 \\
\itshape ${}^*$WGTS Dynamic + SSL & 0.708 & 0.055 & 0.828 & 0.032 \\
\itshape ${}^*$WGTS Dynamic + SSL + dist & \bfseries 0.769 & \bfseries 0.036 & 0.851 & 0.023 \\
\bottomrule
\end{tabular}



